Killing Two Birds with One Stone: Malicious Package Detection in NPM and PyPI using a Single Model of Malicious Behavior Sequence

Open-source software (OSS) supply chain enlarges the attack surface, which makes package registries attractive targets for attacks. Recently, package registries NPM and PyPI have been flooded with malicious packages. The effectiveness of existing malicious NPM and PyPI package detection approaches is hindered by two challenges. The first challenge is how to leverage the knowledge of malicious packages from different ecosystems in a unified way such that multi-lingual malicious package detection can be feasible. The second challenge is how to model malicious behavior in a sequential way such that maliciousness can be precisely captured. To address the two challenges, we propose and implement Cerebro to detect malicious packages in NPM and PyPI. We curate a feature set based on a high-level abstraction of malicious behavior to enable multi-lingual knowledge fusing. We organize extracted features into a behavior sequence to model sequential malicious behavior. We fine-tune the BERT model to understand the semantics of malicious behavior. Extensive evaluation has demonstrated the effectiveness of Cerebro over the state-of-the-art as well as the practically acceptable efficiency. Cerebro has successfully detected 306 and 196 new malicious packages in PyPI and NPM, and received 385 thank letters from the official PyPI and NPM teams.

==> src/ch02-background.tex <==
% !TeX root = ../main.tex

\section{Background}\label{sec:background}

In this section, we discuss the characteristics of the open-source software supply chain attacks. Then, we focus on PyPI and NPM to explore its unique characteristics on malware detection.

\subsection{OSS Supply Chain Attacks}

With the exponential growth of the open-source software (OSS) community, the frequency and impact of attacks targeting the OSS supply chain have reached unprecedented levels. According to predictions by industry experts\cite{gartnerpredict}, it is estimated that nearly half of all organizations worldwide will experience an OSS supply chain attack by the year 2025. This alarming trend can be attributed to several factors, including the vastness of the OSS ecosystem and its loosely-organized developer community.

Package registries have become prime targets for supply chain attacks. Malicious actors exploit vulnerabilities in the OSS supply chain, injecting malicious code or compromising legitimate packages to distribute malware, steal sensitive information, etc. As the battleground has shifted to the OSS domain, it is crucial to understand the underlying reasons for the prevalence of supply chain attacks in platforms like PyPI and NPM. By examining the characteristics of it, we can develop effective countermeasures to safeguard the trustworthiness of the OSS ecosystem.

% With the growing scale of open source software (OSS) community, the attacks to through OSS supply chain are also reaching its historical momentum. It is predicted that nearly half the organizations worldwide will suffer from OSS supply chain attack by the year of 2025\cite{gartnerpredict}. The battleground has shifted to the open source software which is vast and managed by loosely-organized developers. We review the characteristics of adopting OSS and summarize the reason which potentially leads to the prevalence of OSS supply chain attack, especially in PyPI and NPM.

\textbf{Expanded attack surface.} The OSS ecosystem heavily relies on code reuse. While this approach enhances development efficiency, it also significantly expands the attack surface. As highlighted by Zimmermann et al.\cite{zimmermann2019small}, each direct dependency of an NPM package, on average, introduces 79 additional packages and 39 maintainers, providing attackers with a wide range of potential targets. Attackers can exploit vulnerabilities within any of the packages or target the weaknesses of individual maintainers, thereby greatly amplifying the likelihood of a successful attack. This expanded attack surface increases the challenges of ensuring the security and trustworthiness of the open-source software supply chain.

% \textbf{Expanded attack surface.} Open source software is facilitated by code reuse by building its software on numerous dependencies which are included directly and transitively. It improves the efficiency for developing but also introduces the attack surface to a large extent. According to Zimmermann et al.\cite{zimmermann2019small}, a direct dependency of a NPM package transitively introduces 79 packages and 39 maintainers on average, which provides the attackers multiple targets to choose from. Attackers can exploit the vulnerabilities of any of the packages or the weakness of any of the package maintainers, amplifying the attack success rate to a large extent.

\textbf{Automation package manager mechanisms.} The package managers are used in conjunction with the package registries. Modern package managers automate various tasks.
However, this automation can also introduce vulnerabilities and challenges. One key aspect is their ability to resolve and install transitive dependencies transparently for the users of OSS packages. Furthermore, package managers such as \textit{pip} and \textit{npm} typically determine the package version to be installed based on their predefined dependency resolution algorithms. While this mechanism streamlines the process of updating packages, it can be exploited by attackers to conduct covert and continuous malicious activities. Users may remain unaware of the specific versions and dependencies being pulled into their projects, inadvertently introducing vulnerabilities or malicious code.


\textbf{Inadequate security measures.} Open source software fosters collaboration and distribution, but the emphasis on security measures often remains inadequate. The scarcity of human resources within OSS projects can result in inadequate security concerns. Developers may lack the necessary expertise or time to thoroughly address potential vulnerabilities, leaving the downstream consumers exposed to risks. In some cases, project maintainers may bring in new collaborators to share the workload. However, the inclusion of new collaborators introduces additional risks, as their trustworthiness and security practices may not be well-established. Attackers can take advantage of the lax security commitments and the distributed nature of the open-source community, potentially compromising the security and integrity of downstream systems.


%% \textbf{Dynamic languages.} Dynamic languages, such as Python and JavaScript, are commonly used in open source software development. Python and JavaScript interpreters provide a lot of base libraries such as network libraries, encoding/decoding libraries, etc. Further, the programme composed with dynamic languages do not require the compilation process in a new environment. Therefore, it is easier to inject and execute the payload in dynamic languages for attackers.

\textbf{Easy distribution on multiple package registries.} Distribution across multiple packages registries is easy. The attackers can effortlessly devise a malicious skeleton and implement as malicious packages into multiple package registries. In fact, the Sonatype\cite{sonatypereportcryptominers} found that some malicious PyPI and NPM packages share the same author. By looking into the Cryptominers in PyPI and NPM, they confirmed that the Python packages contain identical code to the one seen in npm packages, and the same \textit{https://bit.ly} URL being used to fetch content from remote. This alarming discovery suggests a growing trend of malware translation across languages and a surge in attacks on multiple package registries.


\subsection{PyPI and NPM}

 The Python Package Index (PyPI)\cite{pypi} and NPM\cite{npmjs} are widely recognized as the primary package registries for hosting Python and JavaScript packages, respectively. To facilitate the package management process, PyPI integrates seamlessly with the \textit{pip} package manager, which is the default package manager for Python. Developers can utilize \textit{pip} to upload their packages to PyPI. Similarly, NPM serves as the package registry for JavaScript packages and is closely integrated with the \textit{npm} package manager. Once uploaded and published, packages become publicly available on the respective package registries. Downstream developers can then leverage the package managers to conveniently download and install the desired packages for use in their own projects.

 \textbf{Dynamic languages in Package Management.} Package management in dynamic languages, such as Python and JavaScript, introduces additional complexities and risks compared to package managers for compiled languages like Maven for Java. For instance, in the case of PyPI packages, \textit{pip} automatically executes the \texttt{setup.py} script present at the root of the package during the installation process. This script is responsible for performing any necessary preparations or configurations required for the package installation. Similarly, NPM introduced a mechanism that utilizes \textit{script} property in \textit{package.json}\cite{npmpackagejson}. This property allows developers to specify certain keys, such as \textit{preinstall} or \textit{postinstall} along with corresponding values indicating the paths of scripts to be automatically executed. Further, when a downstream package includes an \textit{import} statement in Python (or a \textit{require} statement in JavaScript) to import a module from a dependency, the corresponding initialization file \texttt{\_\_init\_\_.py} (or \texttt{index.js}/\texttt{index.node} in JavaScript) is executed by default. While dynamic features facilitate the developers, they bring more risk associated with package management. Proper understanding of these dynamic language features is crucial to ensure the security and stability of the package management process.


 \textbf{Malicious Package Datasets.} The PyPI and NPM package repositories have faced numerous security challenges. In 2022, the PyPI team reported removing over \todo{12,000} packages\cite{pypiteammalwarereport}, which are instances of spam, typosquatting, dependency confusion, exfiltration, or malware. Similarly, the Sonatype team identified over \todo{422} malicious packages\cite{sonatypereport}, mostly data exfiltration through typosquatting or dependency confusion attacks in December, 2022. While these numbers highlight the severity of the issue, it is understandable that the PyPI and NPM teams would not openly release the entire collection of malicious packages for preventing potential misuse or exploitation by malicious actors. As a result, the publicly available datasets are relatively limited in size. For our research purposes, we collected a dataset comprising \todo{1,789} malicious NPM packages and \todo{517} malicious PyPI packages, which are smaller than the reported cases. However, the size of the malicious PyPI dataset is relatively smaller than the malicious NPM dataset, which is inconsistent to that in reported numbers. These limitations in dataset availability emphasize the challenges in studying and implementing an effective malicious package detector. Nonetheless, the collected samples provide valuable insights and can contribute to the understanding of the security landscape in malicious packages in package registries.


